Towards the Artificial Brain: A Base Framework for Modelling Consciousness and Unconsciousness

One of the current AI issues depicted in popular culture is the fear of conscious super AIs that try to take control over humanity. And as computational power goes upwards and that turns more and more into a reality, understanding artificial brains might be increasingly important to control and drive AI towards the benefit of our societies. This paper proposes a base framework to aid the development of autonomous multipurpose artificial brains. To approach that, we propose to first model the functioning of the human brain by reflecting and taking inspiration from the way the body, the consciousness and the unconsciousness interact. To do that, we tried to model events such as sensing, thinking, dreaming and acting, thoughtfully or unconsciously. We believe valuable insights can already be drawn from the analysis and critique of the presented framework, and that it might be worth implementing it, with or without changes, to create, study, understand and control artificially conscious systems.

==> bib.tex <==
@misc{arteaga,
author = {Arteaga, Mauricio},
booktitle = {New York Public Library},
mendeley-groups = {PhD Thesis/Automatic Layout,PhD Thesis},
title = {{Generative eBook Covers | The New York Public Library}},
url = {https://www.nypl.org/blog/2014/09/03/generative-ebook-covers},
urldate = {2020-02-24},
year = {2014}
}

@misc{eveillard_2015, title={Portfolio de Louis Eveillard | Couvertures génératives}, url={https://www.louiseveillard.com/projets/couvertures-generatives}, journal={Louiseveillard.com}, author={Eveillard, Louis}, year={2015} }

‌@misc{cruz, title={Data Book Covers}, url={https://cdv.dei.uc.pt/data-book-covers/}, journal={CDV Lab}, author={Cruz, Pedro and Machado, Penousal and João Bicker}, year={2010}, month={Jul}}

@misc{duro, title={Graphic Narratives}, url={https://cdv.dei.uc.pt/graphic-narratives/}, journal={CDV Lab}, author={Duro, Lígia and Machado, Penousal and Rebelo, Artur}, year={2013}, month={Mar}}

@inproceedings{jarebelo2020a,
author = {Jos\'{e} Rebelo and S\'{e}rgio Rebelo and Artur Rebelo},
booktitle = {Joint Proceedings of the ICCC 2020 Workshops (WS 2020)},
editor = {Kreminski, Max and Eisenstadt, Viktor and Pinto, Sofia and Kutz, Oliver},
title = {Experiments in Algorithmic Design of Web Pages},
year = {2020}}

@inproceedings{feiner,
  title={A grid-based approach to automating display layout},
  author={Feiner, Steven},
  booktitle={Proc. Graphics Interface},
  volume={88},
  pages={192--197},
  year={1988}
}

@mastersthesis{ferreira,
  title={Design Editorial Algor{\'\i}tmico},
  author={Ferreira, Diogo and others},
  year={2019},
  school={Universidade de Coimbra}
}

@article{jacobs,
  title={Adaptive document layout},
  author={Jacobs, Charles and Li, Wil and Schrier, Evan and Bargeron, David and Salesin, David},
  journal={Communications of the ACM},
  volume={47},
  number={8},
  pages={60--66},
  year={2004},
  publisher={ACM New York, NY, USA}
}

@article{cleveland,
title = "Style based automated graphic layouts",
journal = "Design Studies",
volume = "31",
number = "1",
pages = "3 - 25",
year = "2010",
issn = "0142-694X",
doi = "https://doi.org/10.1016/j.destud.2009.06.003",
url = "http://www.sciencedirect.com/science/article/pii/S0142694X09000453",
author = "Paul Cleveland",
keywords = "generative design, design automation, graphic design, style, aesthetics",
}

@misc{klein,
author = {Klein, D.},
title = {Evolving Layout: next generation layout tool},
url = {evolvinglayout.com},
urldate = {December 17, 2018},
year = {2016},
note= {Last accessed 17 Dec 2018}
}

@article{geigel,
author = {Geigel, Joe and Loui, Alexander},
title = {Using Genetic Algorithms for Album Page Layouts},
year = {2003},
issue_date = {October 2003},
publisher = {IEEE Computer Society Press},
address = {Washington, DC, USA},
volume = {10},
number = {4},
issn = {1070-986X},
url = {https://doi.org/10.1109/MMUL.2003.1237547},
doi = {10.1109/MMUL.2003.1237547},
journal = {IEEE MultiMedia},
month = oct,
pages = {16–27},
numpages = {12}
}


@inproceedings{rebeloTypePosters,
author = {Rebelo, S{\'e}rgio and Fonseca, Carlos M and Bicker, Jo{\~a}o and Machado, Penousal},
booktitle = {6th Conference on Computation, Communication, Aesthetics and X},
title = {{Experiments in the development of typographical posters}},
year = {2018},
publisher={Universidade do Porto},
address={Porto, Portugal},
}

@inproceedings{Kitamura,
author={S. {Kitamura} and H. {Kanoh}},
booktitle={2011 Fourth International Symposium on Computational Intelligence and Design},
title={Developing Support System for Making Posters with Interactive Evolutionary Computation},
year={2011},
volume={1},
number={},
pages={48-51},
doi={10.1109/ISCID.2011.21},
ISSN={null},
month={Oct},
publisher={IEEE},
address = { Piscataway, USA}
}


@phdthesis{onduygu,
author = {{\"{O}}nduygu, Deniz Cem},
mendeley-groups = {PhD Thesis/Automatic Layout/Graphic Design},
school = {Sabanci University},
title = {{Graphagos: evolutionary algorithm as a model for the creative process and as a tool to create graphic design products}},
url = {https://research.sabanciuniv.edu/24145/ https://www.graphagos.com/portfolio/},
year = {2010}
}

@inproceedings{sorn,
author={D. {Sorn} and S. {Rimcharoen}},
booktitle={2013 International Computer Science and Engineering Conference (ICSEC)},
title={Web page template design using interactive genetic algorithm},
year={2013},
volume={},
number={},
pages={201-206},
keywords={genetic algorithms;hypermedia markup languages;Internet;Web design;Web page template design;interactive genetic algorithm;Web sites;Internet;Web page creation;Web application;HTML files;CSS style sheets;user preferential criteria;score-rules design;Web pages;Genetic algorithms;Sociology;Statistics;Layout;Biological cells;Containers;interactive genetic algorithm;website design;web site design;webpage design;web page template;web template design},
doi={10.1109/ICSEC.2013.6694779},
ISSN={null},
month={Sep.},}

@inproceedings{oliver,
    author = {A. Oliver and N. Monmarch and G. Venturini},
    title = {Interactive Design Of Web Sites With A Genetic Algorithm},
    booktitle = {IN PROCEEDINGS OF THE IADIS INTERNATIONAL CONFERENCE WWW/INTERNET},
    year = {2002},
    pages = {355--362},
    publisher = {}
}

@inproceedings{rebeloMovingPosters,
author={S. Rebelo and Martins, P. and Bicker, J. and Penousal Machado },
title={Using Computer Vision Techniques for Moving Poster Design},
booktitle={6.º Conferência Internacional Ergotrip Design},
year=2017,
publisher={UA Editora},
address={Aveiro, Portugal},
}

@inproceedings{lok,
author = {Lok, Simon and Feiner, Steven and Ngai, Gary},
title = {Evaluation of Visual Balance for Automated Layout},
year = {2004},
isbn = {1581138156},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
doi = {10.1145/964442.964462},
booktitle = {Proceedings of the 9th International Conference on Intelligent User Interfaces},
pages = {101–108},
numpages = {8},
keywords = {visual balance, automated layout},
location = {Funchal, Madeira, Portugal},
series = {IUI ’04}
}

@inproceedings{Harrington,
author = {Harrington, Steven J. and Naveda, J. Fernando and Jones, Rhys Price and Roetling, Paul and Thakkar, Nishant},
title = {Aesthetic Measures for Automated Document Layout},
year = {2004},
isbn = {1581139381},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1030397.1030419},
doi = {10.1145/1030397.1030419},
abstract = {A measure of aesthetics that has been used in automated layout is described. The approach combines heuristic measures of attributes that degrade the aesthetic quality. The combination is nonlinear so that one bad aesthetic feature can harm the overall score. Example heuristic measures are described for the features of alignment regularity separation balance white-space fraction white-space free flow proportion uniformity and page security.},
booktitle = {Proceedings of the 2004 ACM Symposium on Document Engineering},
pages = {109–111},
numpages = {3},
keywords = {aesthetics, document, layout},
location = {Milwaukee, Wisconsin, USA},
series = {DocEng '04}
}

@article{mcmanus,
  title={Arnheim's Gestalt theory of visual balance: Examining the compositional structure of art photographs and abstract images},
  author={McManus, IC and St{\"o}ver, Katharina and Kim, Do},
  journal={i-Perception},
  volume={2},
  number={6},
  pages={615--647},
  year={2011},
  publisher={SAGE Publications Sage UK: London, England}
}

@inproceedings{lopes2022evodesigner,
author = {Daniel Lopes and
Jo{\~{a}}o Correia and
Penousal Machado},
editor = {Tiago Martins and
Nereida Rodr{\'{\i}}guez{-}Fern{\'{a}}ndez and
S{\'{e}}rgio M. Rebelo},
title = {EvoDesigner: Towards Aiding Creativity in Graphic Design},
booktitle = {Artificial Intelligence in Music, Sound, Art and Design – 11th International
Conference, EvoMUSART 2022, Held as Part of EvoStar 2022, Madrid,
Spain, April 20-22, 2022, Proceedings},
series = {Lecture Notes in Computer Science},
volume = {13221},
pages = {162–178},
publisher = {Springer},
address={Berlin, Heidelberg},
year = {2022},
doi = {10.1007/978-3-031-03789-4\_11},
timestamp = {Fri, 22 Apr 2022 19:18:40 +0200},
biburl = {https://dblp.org/rec/conf/evoW/LopesCM22.bib},
bibsource = {dblp computer science bibliography, https://dblp.org}
}

@ARTICLE{neat,
  author={Stanley, Kenneth O. and Miikkulainen, Risto},
  journal={Evolutionary Computation}, 
  title={Evolving Neural Networks through Augmenting Topologies}, 
  year={2002},
  volume={10},
  number={2},
  pages={99-127},
  doi={10.1162/106365602320169811}}

@article{machadoNevar,
author = {Machado, P. and Cardoso, A.},
title = {All the truth about {NEvAr}},
Journal = {Applied Intelligence, Special Issue on Creative Systems},
Editor = {Bentley, P. and Corne, D.},
publisher = {Kluwer Academic publishers},
Volume = {16},
Number = {2},
pages = {101-119}, year = {2002}
}

@inproceedings{martins,
author = {Martins, Tiago and Correia, Jo{\~{a}}o and Costa, Ernesto and Machado, Penousal},
booktitle = {Proceedings of the Genetic and Evolutionary Computation Conference 2016},
organization = {ACM},
pages = {261--268},
title = {{Evotype: from shapes to glyphs}},
year = {2016}
}

@inproceedings{lopes2023evodesigner,
author = {Daniel Lopes and Jo{\~{a}}o Correia and Penousal Machado},
booktitle = {(to be published in) Artificial Intelligence in Music, Sound, Art and Design – 12th International Conference, EvoMUSART 2023, Held as Part of EvoStar 2023, Brno, Czech Republic, April 12-14, 2023, Proceedings},
editor = {Colin Johnson and Nereida Rodr{\'{\i}}guez{-}Fern{\'{a}}ndez and S{\'{e}}rgio M. Rebelo},
publisher = {Springer},
title = {EvoDesigner: Aiding the exploration of innovative graphic design solutions},
year = {2023}}

@article{Zheng,
author = {Zheng, Xinru and Qiao, Xiaotian and Cao, Ying and Lau, Rynson W. H.},
title = {Content-Aware Generative Modeling of Graphic Design Layouts},
year = {2019},
issue_date = {July 2019},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {38},
number = {4},
issn = {0730-0301},
url = {https://doi.org/10.1145/3306346.3322971},
doi = {10.1145/3306346.3322971},
journal = {ACM Trans. Graph.},
month = jul,
articleno = {133},
numpages = {15},
keywords = {deep generative networks, layout, content-aware, graphic design}
}

@ARTICLE{Donovan,
  author={O’Donovan, Peter and Agarwala, Aseem and Hertzmann, Aaron},
  journal={IEEE Transactions on Visualization and Computer Graphics}, 
  title={Learning Layouts for Single-PageGraphic Designs}, 
  year={2014},
  volume={20},
  number={8},
  pages={1200-1213},
  doi={10.1109/TVCG.2014.48}}

@incollection{gans,
title = {Generative Adversarial Nets},
author = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {2672--2680},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5423-generative-adversarial-nets.pdf}
}

@inproceedings{transformers,
 author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, \L ukasz and Polosukhin, Illia},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {I. Guyon and U. Von Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Attention is All you Need},
 volume = {30},
 year = {2017}
}

@incollection{bentley,
author = {Bentley, Peter J. and Corne, David W.},
title = {Introduction to Creative Evolutionary Systems},
booktitle = {Creative Evolutionary Systems},
editor = {Bentley, Peter J. and Corne, David W.},
year = {2002},
isbn = {1-55860-673-4},
pages = {1--75},
numpages = {75},
url = {http://dl.acm.org/citation.cfm?id=510349.510350},
acmid = {510350},
publisher = {Morgan Kaufmann Publishers Inc.},
address = {San Francisco, CA, USA},
}
